Neural Language Modeling with Visual Features

Multimodal language models attempt to incorporate non-linguistic features for the language modeling task. In this work, we extend a standard recurrent neural network (RNN) language model with features derived from videos. We train our models on data that is two orders-of-magnitude bigger than datasets used in prior work. We perform a thorough exploration of model architectures for combining visual and text features. Our experiments on two corpora (YouCookII and 20bn-something-something-v2) show that the best performing architecture consists of middle fusion of visual and text features, yielding over 25% relative improvement in perplexity. We report analysis that provides insights into why our multimodal language model improves upon a standard RNN language model.

==> related.tex <==
\section{Related Work}

Multimodal Language Models were introduced in \cite{kiros2014multimodal}, where log-linear LMs \cite{mnih2007three} where conditioned to handle both image and text modalities. Notably, this work does not use the recurrent neural model paradigm which has now become the \emph{de facto} way of implementing neural LMs.

The community has generally used datasets such as MS COCO \cite{lin2014microsoft} and Flickr \cite{rashtchian2010collecting} for image-based tasks, while several datasets \cite{chen2011collecting,yeung2014videoset,das2013thousand,rohrbach2013translating,hendricks2017localizing} have been curated for video-based tasks. 
Despite the lack of big datasets, language grounding in images \cite{plummer2015flickr30k,rohrbach2016grounding,socher2014grounded} or videos \cite{regneri2013grounding,lin2014microsoft} has been explored (the latter much less than the former) focusing more on obtaining better word or sentence representations. 

The closest work to ours is that of \citet{ororbia2018visually}, implementing a model similar to our \textit{Early Fusion}. Testing on three languages on the MSCOCO dataset, they show perplexity improvements of around 5--6\%. However, their visual modality is static (image) and the model is trained on an English vocabulary of only 16K words.

%Our work could be related to all vision-language tasks. Possibly the most common are image and video caption or description generation, Visual Question Answering (VQA), video retrieval with natural language, and natural object, event, or moment retrieval from images or video.

%In the speech community, 
%audio-visual ASR started by attempting to exploit visual features from the speaker's mouth \cite{gravier2002asynchrony,dupont2000audio,chen2001audiovisual,kashiwagi2012audio}. More recently, 
%recent end-to-end ASR models have used visual grounding \cite{miao2016open,gupta2017visual,palaskar2018end}, but the visual features are constrained to object and place features, as derived from the output of an object/place recognizer. %Instead, our work uses continuous vectors
%Furthermore, multimodal models have been proposed for speaker identification \cite{tapaswi2012knock,bauml2013semi,hu2015deep,ren2016look} and sentiment analysis \cite{chen2017multimodal}. 

Our work is distinguishable from all previous work with respect to the two dimensions. First, our language and visual data are both temporal and roughly parallel, which allows us to model both of them jointly at every time step. Secondly, the scale of our data and experiments is unprecedented, at least two orders of magnitude larger than any previous work.

\iffalse
\begin{enumerate}
    \item 
    \item T The largest dataset currently available at the academic community is DiDeMo \cite{hendricks2017localizing} which has around $2$M tokens. By contrast, our training set comprises around $1.2$B tokens.
\end{enumerate}
\fi



==> wer-yt.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|cc}
    \toprule
        Model & \vod & \pref \\
    \midrule
        word-only & 25.1 & 13.0 \\
    \midrule
        +video & & \\
        +frame & 25.0 & 12.8 \\
        +video +frame & & \\
        +frame +multitask & 24.8 & 12.8 \\
        +frame +weight & 24.9 & 12.8 \\
        +frame +pretrained & & \\
    \bottomrule    
    \end{tabular}
    \caption{WER results on two internal datasets, when we score the lattices with out language models.}
    \label{tab:wer}
\end{table}
